TAC+: Optimizing Error-Bounded Lossy Compression for 3D AMR Simulations

Today's scientific simulations require significant data volume reduction because of the enormous amounts of data produced and the limited I/O bandwidth and storage space. Error-bounded lossy compression has been considered one of the most effective solutions to the above problem. However, little work has been done to improve error-bounded lossy compression for Adaptive Mesh Refinement (AMR) simulation data. Unlike the previous work that only leverages 1D compression, in this work, we propose an approach (TAC) to leverage high-dimensional SZ compression for each refinement level of AMR data. To remove the data redundancy across different levels, we propose several pre-process strategies and adaptively use them based on the data features. We further optimize TAC to TAC+ by improving the lossless encoding stage of SZ compression to handle many small AMR data blocks after the pre-processing efficiently. Experiments on 10 AMR datasets from three real-world large-scale AMR simulations demonstrate that TAC+ can improve the compression ratio by up to 4.9$\times$ under the same data distortion, compared to the state-of-the-art method. In addition, we leverage the flexibility of our approach to tune the error bound for each level, which achieves much lower data distortion on two application-specific metrics.

==> Table/overall-throughput.tex <==
\begin{tabular}{|c *{7}{|c|c|c} | }
% \toprule
\hline
\multirow{2}{*}{$EB_{abs}$} &
  \multicolumn{3}{c|}{\textbf{Run1\_Z2}} &
  \multicolumn{3}{c|}{\textbf{Run1\_Z3}} &
  \multicolumn{3}{c|}{\textbf{Run1\_Z5}} &
  \multicolumn{3}{c|}{\textbf{Run1\_Z10}} &
  \multicolumn{3}{c|}{\textbf{Run2\_T2}} &
  \multicolumn{3}{c|}{\textbf{Run2\_T3}} &
  \multicolumn{3}{c|}{\textbf{Run2\_T4}} \\ \cline{2-22} 
 &
  {1D} &
  {3D} &
  ours &
  {1D} &
  {3D} &
  ours &
  {1D} &
  {3D} &
  ours &
  {1D} &
  {3D} &
  ours &
  {1D} &
  {3D} &
  ours &
  {1D} &
  {3D} &
  ours &
  {1D} &
  {3D} &
  ours \\ \hline
1E+08 &
  {169} &
  {94} &
  97 &
  {166} &
  {90} &
  94 &
  {161} &
  {76} &
  99 &
  {160} &
  {40} &
  95 &
  {152} &
  {17} &
  76 &
  {143} &
  {2.4} &
  60 &
  {125} &
  {0.4} &
  30 \\ \hline
1E+09 &
  {219} &
  {115} &
  121 &
  {213} &
  {120} &
  127 &
  {208} &
  {109} &
  123 &
  {208} &
  {63} &
  117 &
  {193} &
  {27} &
  91 &
  {184} &
  {3.9} &
  66 &
  {159} &
  {0.5} &
  32 \\ \hline
1E+10 &
  {259} &
  {125} &
  135 &
  {256} &
  {125} &
  136 &
  {253} &
  {117} &
  137 &
  {250} &
  {65} &
  135 &
  {242} &
  {30} &
  102 &
  {229} &
  {4.0} &
  72 &
  {197} &
  {0.5} &
  34 \\ \hline
\end{tabular}

% \begin{tabular}{|c *{7}{|c|c|c} | }
% % \toprule
% \hline
% \multirow{2}{*}{$EB_{abs}$} &
%   \multicolumn{3}{c|}{\textbf{Run1\_Z2}} &
%   \multicolumn{3}{c|}{\textbf{Run1\_Z3}} &
%   \multicolumn{3}{c|}{\textbf{Run1\_Z5}} &
%   \multicolumn{3}{c|}{\textbf{Run1\_Z10}} &
%   \multicolumn{3}{c|}{\textbf{Run2\_T2}} &
%   \multicolumn{3}{c|}{\textbf{Run2\_T3}} &
%   \multicolumn{3}{c|}{\textbf{Run2\_T4}} \\ \cline{2-22} 
%  &
%   {1D} &
%   {3D} &
%   ours &
%   {1D} &
%   {3D} &
%   ours &
%   {1D} &
%   {3D} &
%   ours &
%   {1D} &
%   {3D} &
%   ours &
%   {1D} &
%   {3D} &
%   ours &
%   {1D} &
%   {3D} &
%   ours &
%   {1D} &
%   {3D} &
%   ours \\ \hline
% 1E+08 &
%   {169} &
%   {94} &
%   91 &
%   {166} &
%   {90} &
%   88 &
%   {161} &
%   {76} &
%   93 &
%   {160} &
%   {40} &
%   88 &
%   {152} &
%   {17} &
%   76 &
%   {143} &
%   {2.4} &
%   60 &
%   {125} &
%   {0.4} &
%   30 \\ \hline
% 1E+09 &
%   {219} &
%   {115} &
%   112 &
%   {213} &
%   {120} &
%   114 &
%   {208} &
%   {109} &
%   115 &
%   {208} &
%   {63} &
%   106 &
%   {193} &
%   {27} &
%   91 &
%   {184} &
%   {3.9} &
%   66 &
%   {159} &
%   {0.5} &
%   32 \\ \hline
% 1E+10 &
%   {259} &
%   {125} &
%   122 &
%   {256} &
%   {125} &
%   123 &
%   {253} &
%   {117} &
%   127 &
%   {250} &
%   {65} &
%   120 &
%   {242} &
%   {30} &
%   102 &
%   {229} &
%   {4.0} &
%   72 &
%   {197} &
%   {0.5} &
%   34 \\ \hline
% \end{tabular}

==> Table/throughput_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|cccc|cccc|cccc|cccc|cccc|}
\hline
\multirow{2}{*}{EB\_abs} &
  \multicolumn{4}{c|}{\textbf{Run1\_Z10}} &
  \multicolumn{4}{c|}{\textbf{Run1\_Z2}} &
  \multicolumn{4}{c|}{\textbf{Run2\_T2}} &
  \multicolumn{4}{c|}{\textbf{Run2\_T4}} &
  \multicolumn{4}{c|}{\textbf{Run3\_Z1}} \\ \cline{2-21} 
 &
  \multicolumn{1}{c|}{1D} &
  \multicolumn{1}{c|}{3D} &
  \multicolumn{1}{c|}{TAC} &
  TAC+&
  \multicolumn{1}{c|}{1D} &
  \multicolumn{1}{c|}{3D} &
  \multicolumn{1}{c|}{TAC} &
  TAC+&
  \multicolumn{1}{c|}{1D} &
  \multicolumn{1}{c|}{3D} &
  \multicolumn{1}{c|}{TAC} &
  TAC+ &
  \multicolumn{1}{c|}{1D} &
  \multicolumn{1}{c|}{3D} &
  \multicolumn{1}{c|}{TAC} &
  TAC+ &
  \multicolumn{1}{c|}{1D} &
  \multicolumn{1}{c|}{3D} &
  \multicolumn{1}{c|}{TAC} &
  TAC+ \\ \hline
1E+08 &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{79} &
  77 &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{85} &
  84 &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{71} &
  66 &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{0.32} &
  \multicolumn{1}{c|}{24} &
  24 &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{5.6} &
  \multicolumn{1}{c|}{63} &
  63 \\ \hline
1E+09 &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{94} &
  93 &
  \multicolumn{1}{c|}{55} &
  \multicolumn{1}{c|}{92} &
  \multicolumn{1}{c|}{103} &
  97 &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{85} &
  79 &
  \multicolumn{1}{c|}{53} &
  \multicolumn{1}{c|}{0.39} &
  \multicolumn{1}{c|}{26} &
  26 &
  \multicolumn{1}{c|}{53} &
  \multicolumn{1}{c|}{6.5} &
  \multicolumn{1}{c|}{78} &
  75 \\ \hline
1E+10 &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{53} &
  \multicolumn{1}{c|}{107} &
  102 &
  \multicolumn{1}{c|}{58} &
  \multicolumn{1}{c|}{100} &
  \multicolumn{1}{c|}{111} &
  104 &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{98} &
  87 &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{0.41} &
  \multicolumn{1}{c|}{28} &
  27 &
  \multicolumn{1}{c|}{57} &
  \multicolumn{1}{c|}{7.1} &
  \multicolumn{1}{c|}{91} &
  84 \\ \hline
\end{tabular}

